Minimizing Carbon Footprint for Timely E-Truck Transportation: Hardness and Approximation Algorithm

Carbon footprint optimization (CFO) is important for sustainable heavy-duty e-truck transportation. We consider the CFO problem for timely transportation of e-trucks, where the truck travels from an origin to a destination across a national highway network subject to a deadline. The goal is to minimize the carbon footprint by orchestrating path planning, speed planning, and intermediary charging planning. We first show that it is NP-hard even just to find a feasible CFO solution. We then develop a $(1+\epsilon_F, 1+\epsilon_\beta)$ bi-criteria approximation algorithm that achieves a carbon footprint within a ratio of $(1+\epsilon_F)$ to the minimum with no deadline violation and at most a ratio of $(1+\epsilon_\beta)$ battery capacity violation (for any positive $\epsilon_F$ and $\epsilon_\beta$). Its time complexity is polynomial in the size of the highway network, $1/\epsilon_F$, and $1/\epsilon_\beta$. Such algorithmic results are among the best possible unless P=NP. Simulation results based on real-world traces show that our scheme reduces up to 11\% carbon footprint as compared to baseline alternatives considering only energy consumption but not carbon footprint.

==> 3.approach.time.tex <==

\section{A Two-Level Approximation Algorithm}
In this section, we present a two-level approximation algorithm. 
\textcolor{blue}{Give an overview here?}
% At the low-level, we present an algorithm to 

\textbf{Low-level: energy-efficient path from a charging station.} 
We denote by $\Omega(u,v,\tau,\beta_0)$ the maximum achievable SoC from $u$ to $v$ with initial SoC $\beta_0$ and traveling time upper bounded by $\tau$.

\input{algs/approx-low.tex}

% \begin{lemma}
%     If Algorithm~\ref{alg:appro-low} returns NULL, then the parameters $(T_0,\beta_0)$ is infeasible.
% \end{lemma}

\textcolor{blue}{TODO: This Lemma might not be necessary...}
\begin{lemma}
    For any node $u,v \in V$, time upper bound $T_0$, we denote by $\beta^*$ the actual maximum achievable SoC from $u$ to $v$ with initial SoC $\beta_0$ and travel time upper bound $T_0$. If $\beta^*\geq 0$, then $\Omega(u,v, (1+\epsilon)T_0, \beta_0)$ computed from Algorithm~\ref{alg:appro-low} and its corresponding solution $(\vec{p}, \vec{t})$ satisfy the following conditions:
    % If the parameters $(T_0, \beta_0)$ is theoretically feasible, then Algorithm~\ref{alg:appro-low} must return a non-empty solution $(\vec{p},\vec{t})$ such that the total traveling time is less than $(1+\epsilon)T_0$ and final SoC at destination $d$ is larger than maximum achievable SoC $\beta^*$ with deadline $T_0$. That is
    \begin{align}
        \sum_{i=1}^{n} t_i & \leq (1+\epsilon) T_0, \\
        \beta^* & \leq \Omega(u,v,(1+\epsilon)T_0, \beta_0).
    \end{align}
\end{lemma}

% \begin{lemma}[Time Complexity of Algorithm~\ref{alg:appro-low}]
\begin{lemma}
    The time complexity of Algorithm~\ref{alg:appro-low} is $O\left( ( \frac{|V|}{\epsilon} + |V| )^2 |E| \right)$ assuming a constant evaluation time of function $c_e(t)$.
\end{lemma}


\textbf{High-level: routing and planning for charging.}


We define $\rho(s,v,\tau, \beta_0)$ as the minimum objective from the node $s$ to the node $v$ with initial SoC $\beta_0$ and the travel time upper bounded by $\tau$.

\input{algs/approx-high.tex}

\begin{theorem}
    If the parameters of the CFO problem are theoretically feasible, then Algorithm~\ref{alg:appro-high} must return a solution profile $(\vec{p}, \vec{t}^r, \vec{t}^w, \vec{t}^c)$ such that
    \begin{align}
        \sum_{i=1}^{n} t^r_i + \sum_{i=1}^{m} (t^w_i + t^c_i) \leq (1+\epsilon) T \\
        F(\vec{p}, \vec{t}^r, \vec{t}^w, \vec{t}^c) \leq (1+\epsilon L T) \text{OPT}
    \end{align}
    where OPT is the optimal objective of the CFO problem.
\end{theorem}

\begin{theorem}
    The time complexity of Algorithm~\ref{alg:appro-high} is ...
    % $O\left( ( \frac{|V|}{\epsilon} + |V| )^2 |E| \right)$ assuming a constant evaluation time of function $c_e(t)$.
\end{theorem}

% \subsection{Performance Analysis}
% 
% \textbf{Time Complexity.}
% 
% \textbf{}

==> algs/approx-high-soc.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{apxTest$(s, d, T, \Omega, \epsilon_\beta, \epsilon_F)$ \textcolor{blue}{Too long, need to simplify} }\label{alg:appro-high-soc-test}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        \State $\delta_\beta \gets \frac{\epsilon_\beta B}{|V|+1}$, 
        ${M}_{\beta} \gets \lceil \frac{|V|+1}{\epsilon_\beta} \rceil + |V| + 1$
        \State $\delta_F \gets \frac{\epsilon_F \Omega}{|V|+1}$, $M_F \gets \lceil \frac{|V|+1}{\epsilon_F}\rceil + |V| + 1 $
        \State $\hat{\beta_0} \gets \lfloor (1+\epsilon_\beta) B / \delta \rfloor \cdot \delta $
        \State $\psi \gets $ NULL
        \For{$i \gets [0,1,...,M_\beta ], v \in V_c \cup \{s,d\}$ }
            \State $\psi' \gets \text{getMinT}(v,B,i\delta_\beta, \epsilon_\beta)$ 
            \State $\psi \gets \text{merge}(\psi', \psi)$
        \EndFor
        \State $\sigma(s,s,\cdot, \cdot, \cdot) \gets 0$
        \State $\sigma(s,v,\cdot, \cdot, \cdot) \gets \infty, \forall v \in V \backslash \{s\}$

        % \For{$i_c \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        % $i_v \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        % $i_{ini} \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,}
        \For{$i_c \gets [M_\beta, M_\beta -1, ..., 0]$,
             $i_v \gets [M_\beta, M_\beta -1, ..., 0]$,
             $i_w \gets [M_\beta, M_\beta -1, ..., 0]$,
        }
        % $i_v \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,
        % $i_{ini} \gets \overline{M}_{\beta} \text{ to } \underline{M}_{\beta}$,}
 
        \For{$i_\rho \gets 1 \text{ to } M_F$,\, $i_F \gets 1 \text{ to } M_F$}
        \For{$u\in V_c \cup \{s\},\, v \in V_c \cup \{d\}$}
            \State $\rho \gets i_\rho \delta_F$, 
            $\beta_v \gets i_v \delta_\beta$,
            $\hat{F} \gets i_F \delta_F$, 
            $\beta_{ini} \gets i_{ini} \delta_{\beta}$

            \If{$u=s$}
                \State $\beta_{ini} \gets \hat{\beta}_0$
            \EndIf



            \State $\sigma_u \gets \sigma(s, u, \rho, \hat{\beta}_0, \beta_{ini}) $
            \If{$u \notin V_c$}
                \State $\beta_c \gets 0 $,
                $t_w \gets 0$,
                % $t_c \gets 0$
            \Else
                \State $\beta_c \gets i_c \delta_\beta$
                % \State $\tau_u \gets \psi(s, u, \hat{\beta}_0, \beta_{ini})$
                \State $t_w \gets g_v(\beta_{ini}, t_c, \sigma_u, \hat{F})$
            \EndIf
            % \State $t_c \gets \phi^{-1}(\beta_{ini}, \beta_c)$

            \State $\beta_u' = \min\{B, \beta_{ini} + \beta_c\}$
            \State \Longunderstack{$t_c \gets \Phi_u^{-1}( \beta_u' ) - \Phi_u^{-1}(\beta_{ini})$}
            \State $t_r \gets \psi(u,v, \beta_u', \beta_v)$

            \State $\tilde{\sigma} \gets \sigma_u + t_r + t_w + t_c $
            \State $\sigma_v \gets \sigma(s, v, \rho + \hat{F}, \hat{\beta}_0, \beta_v) $
            \If{ $\tilde{\sigma} \leq \sigma_v$ }
                \State $\sigma(s, v, \rho+\hat{F}, \hat{\beta}_0, \beta_v) \gets \tilde{\sigma}$
            \EndIf
        \EndFor
        \EndFor
        \EndFor
        % $\text{sol} \gets \text{NULL}$, 
        

        \State Let $i^*_\rho \in \left\{ 0,\cdots, M \right\}$ be the minimal $i_\rho$ such that $\sigma(s, d, i_\rho \delta_F, \hat{\beta}_0, 0 ) \leq T $
        \If{$\rho^*$ exists}
            \State sol $\gets$ the solution corresponding to $\rho^*$
        \Else
            \State sol $\gets$ NULL
        \EndIf
        \State \Return sol
        
    \end{algorithmic}
\end{algorithm}

==> algs/approx-high.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{solveCFO$(s,d,T,\beta_0, \epsilon)$ \textcolor{blue}{Not ready yet. This form of algorithm might be wrong...}}\label{alg:appro-high}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        \State 
        % $\text{sol} \gets \text{NULL}$, 
        $\delta\gets\frac{\epsilon T}{|V|+1}$, $M\gets\lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1$
        \State $\rho(s,s, i\delta, \beta_0) \gets 0, \forall i \in \left\{ 1,...,M \right\}$
        \State $\rho(s,v, i\delta, \beta_0) \gets \infty, \forall i \in \left\{ 1,...,M \right\}, \forall v \in V \backslash \{s\}$
        \State $\beta_s \gets \beta_0$
        \State $\beta_v \gets -\infty, \forall v \in V \backslash \{s\}$
        \For{$i_c \gets 1$ to $M$, $i_w \gets 1$ to $M$, $i_{r} \gets 1$ to $M$, $i_{\tau} \gets 1$ to $M$}
            \State $t_c \gets i_c\delta,\, t_w \gets i_w\delta $
            \State $t_r \gets i_c\delta,\, \tau \gets i_{\tau}\delta $
            \If{$t_c \in [0, t_c^{ub}+\delta]$ and $t_w \in [t_w^{lb}, t_w^{ub}+\delta]$}
            \State $t_c \gets \min \left\{ t_c, t_c^{ub} \right\}$, $t_w \gets \min \left\{ t_w, t_w^{ub} \right\}$
            \For{$u \in \{s,d\} \cup V_c,\, v \in \{s,d\} \cup V_c $}
                \State $\tilde{\rho} \gets \rho(s, u, \tau, \beta_0) + F_u(\beta_u, t_c, \tau+t_w)$
                \State $\rho_{prev} \gets \rho(s, v, \tau + t_c + t_w + t_r)$
                \State { \Longunderstack[l]{$\tilde{\beta}\gets\beta(u,v,t_r,\beta_u+\phi(t_c,\beta_u))$ \\\; computed by calling Algorithm~\ref{alg:appro-low} \\\; with the same parameters and tolerance $\epsilon$}}.
                \If{$\tilde{\rho} < \rho_{prev} $ and $\tilde{\beta}\geq 0$}
                    \State $\rho(s,v,\tau+t_c+t_w,t_r) \gets \tilde{\rho}$
                    \State $\beta_v \gets \tilde{\beta}$
                \EndIf
                % \If{$t_e \in [t_e^{lb}, t_e^{ub}]$ }
                %     \State $\tilde{\beta} \gets \min\left\{ B, \beta(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                %     \If{$\tilde{\beta} \geq 0$}
                %         \State \Longunderstack[l]{$\beta(s,v,\tau+t_e,\beta_0)=$
                %         $\qquad\max\left\{\tilde{\beta},\beta(s,v,\tau+t_e,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                %         % $  $
                %         }
                %     \EndIf
                % \EndIf
            \EndFor
            \EndIf
        \EndFor

        \If{\textcolor{blue}{TODO:}}
            \State sol $\gets$ the solution for ... % $\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right)$
        \Else
            \State sol $\gets$ NULL
        \EndIf
        \State \Return sol
        
    \end{algorithmic}
\end{algorithm}

==> algs/approx-low-soc.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{getMinT$(s,B_0,\beta_0, \epsilon)$}\label{alg:appro-low-soc}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        % \State \textbf{Initialization Phase:} 
        % $\text{sol} \gets \text{NULL}$, 
        \State $\delta\gets\frac{\epsilon B_0}{|V|+1}$, 
        % $\underline{M}\gets  -(|V| + 1) $, 
        $M \gets \lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1$
        \State $\hat{\beta_0} \gets \lfloor \beta_0 / \delta \rfloor \delta $
        \State  $\psi(s,s, \hat{\beta_0}, i\delta) \gets 0, \forall i \in \left\{ 0,...,M \right\}$
        \State  $\psi(s,v, \hat{\beta_0}, i\delta) \gets \infty, \forall i \in \left\{ 0,...,M \right\}, \forall v \in V \backslash \{s\}$
        \For{$i \gets [M,M-1,...,0 ] $}
            \For{$e = (u,v) \in E$}
                
            \For{$j \gets \lfloor \frac{c^{lb}_e}{\delta} \rfloor \text{ to } \lceil \frac{c^{ub}_e}{\delta} \rceil $}
                
                \State $\beta_u \gets i\delta$, $\hat{c} \gets j\delta$
                \If{$u=s$}
                    \State $\beta_u \gets \hat{\beta}_0$
                \EndIf
                \begin{equation}
                    % \setlength{\mathindent}{0pt}
                    % \hspace{-5mm}
                    t_e \gets \left\{  
                        \begin{aligned}
                            & t_e^{lb},& \text{if } j = \lceil \frac{c_e^{ub}}{\delta} \rceil, \\
                            & c_e^{-1}(\hat{c}), & \text{if } \hat{c} \in [c_e^{lb}, c_e^{ub}),  \\
                            & \infty, & \text{otherwise}.
                        \end{aligned}
                    \right.
                \end{equation}
                \State $\beta_v \gets \min \{(1+\epsilon)B, \beta_u - \hat{c}\}$
                \If{$ \beta_v \in [0, (1+\epsilon) B]$}
                    \State $\tilde{\psi} \gets \psi(s, u, \hat{\beta}_0, \beta_u) + t_e$
                    \State $\psi_{prev} \gets \psi(s, v, \hat{\beta}_0, \beta_v) $
                    \State $\psi(s,v, \hat{\beta}_0, \beta_v) \gets \min \left\{ \tilde{\psi}, \psi_{prev}  \right\}$
                \EndIf
                % \If{$t_e \in [t_e^{lb}, t_e^{ub} + \delta]$ }
                %     \State $t_e \gets \min \left\{ t_e, t_e^{ub} \right\}$
                %     \State $\tilde{\psi} \gets \min\left\{ B, \psi(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                %     \If{$\tilde{\psi} \geq 0$}
                %         \State \Longunderstack[l]{$\psi(s,v,\tau+t_e,\beta_0)\gets$
                %         \\ $\qquad\max\left\{\tilde{\psi},\psi(s,v,\tau+i\delta,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                %         % $  $
                %         }
                %     \EndIf
                % \EndIf
            \EndFor
            \EndFor
        \EndFor

        \State \Return $\psi$
        
    \end{algorithmic}
\end{algorithm}

==> algs/approx-low.tex <==

\begin{algorithm}[!tb]

    % \newcommand{\multiline}[1]{%
    %     \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    %       #1
    %     \end{tabularx}
    % }

    \caption{getMaxSoC$(s,T_0,\beta_0, \epsilon)$}\label{alg:appro-low}
    \begin{algorithmic}[1]
        % \SetInd{0.25em}{0.1em}
        % \State \textbf{Initialization Phase:} 
        % $\text{sol} \gets \text{NULL}$, 
        \State $\delta\gets\frac{\epsilon T_0}{|V|+1}$, $M\gets \left(   \lceil \frac{|V|+1}{\epsilon} \rceil + |V| + 1 \right)$
        \State  $\Omega(s,s, i\delta, \beta_0) \gets \beta_0, \forall i \in \left\{ 1,...,M \right\}$
        \State  $\Omega(s,v, i\delta, \beta_0) \gets - \infty, \forall i \in \left\{ 1,...,M \right\}, \forall v \in V \backslash \{s\}$
        \For{$i \gets 1$ to $M$, $j \gets 1$ to $M$}
            \For{$e = (u,v) \in E$}
                \State $t_e \gets i\delta, \tau \gets j\delta$
                \If{$t_e \in [t_e^{lb}, t_e^{ub} + \delta]$ }
                    \State $t_e \gets \min \left\{ t_e, t_e^{ub} \right\}$
                    \State $\tilde{\Omega} \gets \min\left\{ B, \Omega(s,u, \tau, \beta_0) - c_e(t_e) \right\}$
                    \If{$\tilde{\Omega} \geq 0$}
                        \State \Longunderstack[l]{$\Omega(s,v,\tau+t_e,\beta_0)\gets$
                        \\ $\qquad\max\left\{\tilde{\Omega},\Omega(s,v,\tau+i\delta,\beta_0)\right\}$%$\max\{\tilde{\beta},\beta(s,v,\tau+t_e, \beta_0)\}$
                        % $  $
                        }
                    \EndIf
                \EndIf
            \EndFor
        \EndFor

        % \If{$\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right) \geq 0$}
        %     \State sol $\gets$ the solution for $\beta\left(s,d,(1+\epsilon)T_0,\beta_0\right)$
        % \Else
        %     \State sol $\gets$ NULL
        % \EndIf

        % \For{$k \gets 1$ to $K$}
        %     % \State Compute $\text{sol}^+$ with $\vec{\lambda}[k]$ by solving problem~\eqref{prob:dual} \label{alg:dualsub:primal}
        %     \If{$\delta_i^\beta[k] = 0$ and $\delta_i^\tau[k] = 0, \forall i\in \left\{ 1,...,N+1 \right\}$}
        %         \State \Return sol $\gets \text{sol}^+$  \label{alg:dualsub:optimal}
        %     \EndIf
        %     \If{$\delta_i^\beta[k] \leq 0$ and $\delta_i^\tau[k] \leq 0, \forall i\in \left\{ 1,...,N+1 \right\}$ \textbf{and} $\text{sol}^+$ has less objective }
        %         \State sol $\gets \text{sol}^+$ 
        %     \EndIf
        %     % \State $\hat{p} \gets \text{DFS}(\emptyset, p^\star, n)$
        %     % \If{$g(\hat{p}) < g(p^\star) $}
        %     %     \State $p^\star \gets \hat{p}$
        %     % \State Compute $\vec{\lambda}[k+1]$ according to~\eqref{eq:dualupdate}.
        % \EndFor
        \State \Return $\Omega$
        
    \end{algorithmic}
\end{algorithm}

==> tabs/co2-fuel.tex <==
\begin{table}[tb]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lllll}
        \toprule
        & Coal & Natural gas & Petroleum & Renewable \\
        \midrule
        Carbon Intensity (kg/kWh) & 1.02 & 0.39 & 0.91 & 0 \\
        Total emission (tons) & 7.86 $\times 10^8$ & 6.35 $\times 10^8$& 1.6 $\times 10^7$ & 0\\
        Electricity (kWh) & 7.73 $\times 10^{11}$ & 1.62$\times 10^{12}$ & 1.75 $\times 10^{10}$ & $7.92\times 10^{11}$  \\
        \bottomrule
    \end{tabular}
    } % end of resizebox
    \vspace{1mm}
    \caption{U.S electricity generation and resulting \coo\ emissions by major type of source in 2020~\cite[Tab.~7.2a, Tab.~11.6]{eia2021monthly}}\label{tab:fuel-co2}
    \vspace{-6mm}
    \vspace{6mm}
\end{table}
